Swan and ArabicMTEB: Dialect-Aware, Arabic-Centric, Cross-Lingual, and Cross-Cultural Embedding Models and Benchmarks

We introduce {\bf Swan}, a family of embedding models centred around the Arabic language, addressing both small-scale and large-scale use cases. Swan includes two variants: Swan-Small, based on ARBERTv2, and Swan-Large, built on ArMistral, a pretrained Arabic large language model. To evaluate these models, we propose ArabicMTEB, a comprehensive benchmark suite that assesses cross-lingual, multi-dialectal, multi-domain, and multi-cultural Arabic text embedding performance, covering eight diverse tasks and spanning 94 datasets. Swan-Large achieves state-of-the-art results, outperforming Multilingual-E5-large in most Arabic tasks, while the Swan-Small consistently surpasses Multilingual-E5-base. Our extensive evaluations demonstrate that Swan models are both dialectally and culturally aware, excelling across various Arabic domains while offering significant monetary efficiency. This work significantly advances the field of Arabic language modelling and provides valuable resources for future research and applications in Arabic natural language processing. Our models and benchmark are available at our GitHub page: \href{https://github.com/UBC-NLP/swan}{https://github.com/UBC-NLP/swan}

==> Figures_latex/pipeline.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=1\columnwidth]{Figures/rag.pdf}
\caption{Pipeline showing an example of Embedding models}
\label{fig:Arabic MTEB}
\end{figure}

==> Tables/arabic_inst_data.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table}[!htp]\centering
\scriptsize
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lr}\toprule
\textbf{Source} &\textbf{\#Samples} \\\midrule
Arabic-OpenHermes-2 &981618 \\
Orca &500247 \\
Quora\_QA &247644 \\
Transliteration &209254 \\
GPT4\_instructions &114217 \\
Diacritization &50000 \\
Style transfer &40433 \\
News Title Generation &37519 \\
Summarization &37519 \\
Machine Translation &21758 \\
Mawdoo\_qa &19755 \\
GEC &19411 \\
Question Answering &14805 \\
Question Generation &14805 \\
Aya-cleaned &11548 \\
CIDAR &10000 \\
H4\_no\_robots\_ar &9500 \\
ALP\_ar\_arc\_train &2234 \\
Paraphrasing &2109 \\\midrule
\textbf{Total} &\textbf{2344376} \\
\bottomrule
\end{tabular}}
\caption{Generated by Spread-LaTeX}\label{tab: }
\end{table}

==> Tables/arabic_llm_eval.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table}[!htp]\centering
\scriptsize
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lrrr}\toprule
\textbf{Cluster} &\textbf{Dataset} &\textbf{\#Shots} &\textbf{\#Tasks} \\\midrule
\multirow{3}{*}{Commonsense Reasoning} &HellaSwag &5 & \\
&ARC &25 & \\
&PiQA &5 & \\\midrule
ExtractiveQA &OpenBookQA &0 & \\\midrule
Hate Speech Detection &Toxigen &0 & \\\midrule
\multirow{7}{*}{Multiple-Choice QA} &BoolQ &5 & \\
&SciQA &5 & \\
&ExamsQA &5 &9 tasks \\
&MMLU &5 &57 tasks \\
&TruthfulQA &0 & \\
&AlGhafa &5 &7 tasks \\
&ACVA &5 &56 tasks \\\midrule
NLG &Dolphin &5 &26 tasks \\\midrule
NLU &ORCA &5 &12 tasks \\\midrule
Reading Comprehension &RACE &0 & \\\midrule
Instruction Following &IFEval &0 & \\\midrule
\multirow{4}{*}{LongContext} &NarrativeQA &0 &+RAG \\
&HotpotQA &0 &+RAG \\
&MultiFieldQA &0 &+RAG \\
&PassageRetrieval &0 &+RAG \\\midrule
Case Study &GEC &0 &+RAG \\
\bottomrule
\end{tabular}}
\caption{Generated by Spread-LaTeX}\label{tab: }
\end{table}
